Ternary Hashing

This paper proposes a novel ternary hash encoding for learning to hash methods, which provides a principled more efficient coding scheme with performances better than those of the state-of-the-art binary hashing counterparts. Two kinds of axiomatic ternary logic, Kleene logic and {\L}ukasiewicz logic are adopted to calculate the Ternary Hamming Distance (THD) for both the learning/encoding and testing/querying phases. Our work demonstrates that, with an efficient implementation of ternary logic on standard binary machines, the proposed ternary hashing is compared favorably to the binary hashing methods with consistent improvements of retrieval mean average precision (mAP) ranging from 1\% to 5.9\% as shown in CIFAR10, NUS-WIDE and ImageNet100 datasets.

==> map_linechart_storage.tex <==
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.7\linewidth]{legend.png}
	\\
	\begin{subfigure}[b]{0.4\linewidth}
		\centering
		\includegraphics[width=\linewidth]{bitlength_greedyhash_imagenet100.png}
		\caption{GreedyHash}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\linewidth}
		\centering
		\includegraphics[width=\linewidth]{bitlength_dpn_imagenet100.png}
		\caption{DPN}
	\end{subfigure}

	\caption{Performance against different bit length on ImageNet100.}
	\label{fig:maplinestorage}
\end{figure}
